Domain-Robust Mitotic Figure Detection with Style Transfer

We propose a new training scheme for domain generalization in mitotic figure detection. Mitotic figures show different characteristics for each scanner. We consider each scanner as a 'domain' and the image distribution specified for each domain as 'style'. The goal is to train our network to be robust on scanner types by using various 'style' images. To expand the style variance, we transfer a style of the training image into arbitrary styles, by defining a module based on StarGAN. Our model with the proposed training scheme shows positive performance on MIDOG Preliminary Test-Set containing scanners never seen before.

==> figures/retinanet.tex <==
\adjustbox{max width=0.5\textwidth}{
\begin{tikzpicture}[] 
\tikzstyle{every node}=[trapezium, draw, minimum width=3cm,
trapezium left angle=60, trapezium right angle=120]

% Encoder
\node[draw=none,
           path picture={
               \node at (path picture bounding box.center){
                   \includegraphics[width=4cm]{figures/mf.png}
               };
           }] at (0,-0.75) {};
\node[purple, minimum width = 3cm, fill=white, line width=1.5] (enc0) at (0,0) {};
\node[draw=none, purple, below = 1 cm of enc0, align=center] {ResNet Encoder}; 
\node[purple, minimum width = 2.5cm, fill=white, line width=1.5] (enc1) at (0,0.75) {};
\node[purple, minimum width = 2cm, fill=white, line width=1.5] (enc2) at (0,1.5) {};

% Decoder
\node[teal, minimum width = 3 cm, fill=white, line width=1.5, align = center] (dec0) at (5,0) {};
\node[draw=none, teal, below = 1 cm of dec0, align=center] {Feature Pyramid \\ Network}; 
\draw[->] (5,0.75) -- ($(dec0.center)+ (0,-0.2)$);
\node[teal, minimum width = 2.5cm, fill=white, line width=1.5] (dec1) at (5,0.75) {};
\draw[->] (5,1.5) -- ($(dec1.center)+ (0,-0.2)$);
\node[teal, minimum width = 2cm, fill=white, line width=1.5] (dec2) at (5,1.5) {};

\node[draw=none, align=center] (pred) at (9,0) {class + box \\ subnets};
\draw[->] (dec0.east) -- (pred.west);
\node[draw=none, align=center] (dis) at (0,3) {domain \\ discriminator};


\draw[->] ($(enc0.center)+ (0,-0.2)$) -| (enc1.south);
\draw[->] ($(enc1.center)+ (0,-0.2)$) -| (enc2.south);

\draw[->] (enc0.east) -- (dec0.center);
\draw[->] (enc1.east) -- (dec1.center);
\draw[->] (enc2.east) -- (dec2.center);
\draw[->, rounded corners] (enc2.center)  -- (dis.south);
\end{tikzpicture}}


